FIPA-based Interoperable Agent Mobility Proposal

This paper presents a proposal for a flexible agent mobility architecture based on IEEE-FIPA standards and intended to be one of them. This proposal is a first step towards interoperable mobility mechanisms, which are needed for future agent migration between different kinds of platforms. Our proposal is presented as a flexible and robust architecture that has been successfully implemented in the JADE and AgentScape platforms. It is based on an open set of protocols, allowing new protocols and future improvements to be accommodated in the architecture. With this proposal we demonstrate that a standard architecture for agent mobility capable of supporting several agent platforms can be defined and implemented.

==> sections/interoperability.tex <==
\section{Implementations}
\label{sec:implementations}

The migration architecture presented in this paper has been
successfully implemented and tested in two different agent platforms:
JADE and AgentScape.  In the case of the JADE agent platform, the new
migration architecture is the evolution of the former migration
service~\cite{acmnr0906}. This can be downloaded from the JIPMS
SourceForge project website as from the development release 1.98.  The
proposed migration has also been implemented into the AgentScape
platform, once successfully tested in JADE. This has involved the
implementation of several FIPA specifications because AgentScape is
not a FIPA compliant platform. These implementations prove that the
proposed architecture is valid for completely different agent
platforms.

\begin{table*}
  \centering
  \begin{tabular}{|p{60pt}|p{150pt}|p{50pt}|p{75pt}|}
    \hline
    \multicolumn{1}{|l|}{\textbf{Frame}} &
    \multicolumn{3}{|l|}{push-transfer-protocol-transfer} \\
    \hline
    \multicolumn{1}{|l|}{\textbf{Ontology}} &
    \multicolumn{3}{|l|}{push-transfer-protocol-ontology-v1} \\
    \hline
    \textbf{Parameter}&\textbf{Description}&\textbf{Presence}&\textbf{Type} \\
    \hline
    cid & Agent code unique identifier (CID) & Optional & String \\
    \hline
    code & Agent code & Optional & Byte-Stream \\
    \hline
    data & Agent data & Mandatory & Byte-Stream \\
    \hline
    state & Agent state & Optional  & Byte-Stream \\
    \hline
  \end{tabular}
  \caption{Push Transfer Protocol Ontology: transfer agent.}
  \label{tab:push-transfer-ontology}
\end{table*}

%
%
%
%
%

%


==> sections/supported-protocols.tex <==
\section{Pre-agreement stage}
\label{sec:supported-protocols}

The migration proposal presented on the first section allows an
agent to migrate with a subset of migration protocols. These ones
are chosen by the agent before calling the \texttt{doMove()}, or
whatever similar, method.

But the protocols to use with the destination platform must be known
a priori by the agent. As this is impossible, because the agent
cannot be provided with this information for all platforms of the
world, a method to retrieve it is needed. Then, on this section, we
propose a protocol to retrieve the supported protocols of the
migration service where it belongs to.

The idea is to request the remote platform where the agent is
planning to go, a list of all supported protocols in each of the
steps of the migration architecture.

Asking this list every time an agent wants to migrate is quite
inefficient, thus each implementation is free to develop some kind of
list cache, saving previous queried results.

\subsubsection{Message flow}
\label{sec:supported-protocols-flow}

That protocol uses a FIPA Request Interaction protocol \cite{FIPA026}
(see Figure~\ref{fig:fipa-request}). It starts with a \texttt{request}
message which contains a \texttt{get-supported-protocols} action.

Once the first message is sent, the source platform expects to receive
an \texttt{inform-result} with the list of supported protocols. In
case of error a \texttt{failure} message will be received. The
\texttt{refuse} and \texttt{agree} messages are not needed in this
protocol.

\subsubsection{Ontology}
\label{sec:supported-protocols-ontology}

These protocol use the same ontology of the whole proposal, despite
being used apart of that. Then, an action to ask for the supported
protocols, called \texttt{get-supported-protocols}, is defined (see
Table~\ref{tab:get-supported-protocols-action}). Furthermore a frame
to include the list of supported protocols in the
\texttt{inform-result} message is included (see
Table~\ref{tab:supported-protocols}), which is encapsulated as a
predicate.

\begin{table*}
  \centering
  \begin{tabular}{|p{60pt}|p{260pt}|}
    \hline
    \textbf{Function} & get-supported-protocols \\
    \hline
    \textbf{Ontology} & migration-ontology \\
    \hline
    \textbf{Supported by} & AMM \\
    \hline
    \textbf{Description} & An AMM agent issues a \texttt{get-supported-protocols} request to get the migration supported protocols into the destination platform. \\
    \hline
    \textbf{Domain} & migration-ontology \\
    \hline
    \textbf{Arity} & 1 \\
    \hline
  \end{tabular}
  \caption{Migration Ontology: Get-Supported-Protocols action}
  \label{tab:get-supported-protocols-action}
\end{table*}

\begin{table*}
  \centering
  \begin{tabular}{|p{60pt}|p{150pt}|p{50pt}|p{95pt}|}
    \hline
    \multicolumn{1}{|l|}{\textbf{Frame}} &
    \multicolumn{3}{|l|}{supported-protocols} \\
    \hline
    \multicolumn{1}{|l|}{\textbf{Ontology}} &
    \multicolumn{3}{|l|}{migration-ontology} \\
    \hline
    \textbf{Parameter}&\textbf{Description}&\textbf{Presence}&\textbf{Type} \\
    \hline
    pre-transfer & Pre-transfer protocols accepted & Optional & Set of String \\
    \hline
    transfer & Transfer protocols accepted & Mandatory & Set of String \\
    \hline
    post-transfer & Post-transfer protocols accepted & Optional & Set of String \\
    \hline
  \end{tabular}
  \caption{Migration Ontology: Supported protocols}
  \label{tab:supported-protocols}
\end{table*}

%
%
%
%
%

%

